Automating PTSD Diagnostics in Clinical Interviews: Leveraging Large Language Models for Trauma Assessments

The shortage of clinical workforce presents significant challenges in mental healthcare, limiting access to formal diagnostics and services. We aim to tackle this shortage by integrating a customized large language model (LLM) into the workflow, thus promoting equity in mental healthcare for the general population. Although LLMs have showcased their capability in clinical decision-making, their adaptation to severe conditions like Post-traumatic Stress Disorder (PTSD) remains largely unexplored. Therefore, we collect 411 clinician-administered diagnostic interviews and devise a novel approach to obtain high-quality data. Moreover, we build a comprehensive framework to automate PTSD diagnostic assessments based on interview contents by leveraging two state-of-the-art LLMs, GPT-4 and Llama-2, with potential for broader clinical diagnoses. Our results illustrate strong promise for LLMs, tested on our dataset, to aid clinicians in diagnostic validation. To the best of our knowledge, this is the first AI system that fully automates assessments for mental illness based on clinician-administered interviews.

==> tex/results.tex <==
\section{Results}
\label{sec:results}

\begin{table*}[htbp!]
  \centering \small{ %\resizebox{\columnwith}{!}{
  \begin{tblr}{    
    colspec = {MMMMMMMMMM},
    hline{1, Z} = {1pt, solid},
    hline{2} = {0.5pt, solid},
    hline{3} = {0.7pt, solid}}
    \SetCell[r=2]{c}\bf Type & \SetCell[r=2]{c}\bf Count & \SetCell[c=2]{c}\bf Acc & &\SetCell[c=2]{c}\bf RMSE && \SetCell[c=2]{c}\bf Bias && \SetCell[c=2]{c}\bf Recall &\\
    & &  ChatGPT & Llama2 & ChatGPT & Llama2 & ChatGPT& Llama2 & ChatGPT & Llama2\\
    Scale & 9,722 & 59.2 & 46.7 & 1.09 & 1.25 & 48.0 & 75.7 & - & -\\
    Scale\_group & 9,722 & 67.6 & 59.0 & 0.85 & 1.01 & 48.5 & 75.6 & -& -\\
    Category & 4,258 & 77.2 & 63.6 & - & - & -& - & - & -\\
    Calculation & 3,482 & 64.4 & 56.5 & - & - & 33.0 & 49.8 & -& - \\
    Notes & 1,146 & -& - & -& - & -& - & 48.1& 52.7\\
    Rule\_based & 2,828 & 56.3& & 0.96& & 41.3& & -& - \\
  \end{tblr}}
  \caption{Accuracy, Root Mean Square Error (RMSE), positive Bias Evaluation, and Recall achieved by both models for each variable.}
  \label{tab:results}
\end{table*}


Table~\ref{tab:results} gives the results for each variable type.
For \emph{Scale Variable}, we additionally evaluate it with grouped scales for CAPS-5 question set.
This approach is justified by the nature of CAPS-5 scaling, which ranges from 0 to 4. 
A score of 0 indicates the absence of symptoms, a score of 1 denotes minimal symptoms, and scores above 2 are considered as symptoms that meet or exceed the threshold for clinical significance. 
Therefore, to reflect this clinical demarcation, scale points were categorized into three scale groups.

ChatGPT consistently shows superior performance by an average of 10\% across most metrics and variable types.
However, Llama2 displays a higher recall for \emph{Note Variables}. 
Specifically, for \emph{Scale Variable}, ChatGPT demonstrates a higher accuracy (59.2) compared to Llama2 (46.7).
Additionally, ChatGPT shows a more favorable RMSE (1.09 vs. 1.25), indicating a closer proximity to the gold data.
However, ChatGPT tends to be more conservative when predicting the answer with a positive Bias of 48.0, whereas Llama2 is more likely to overestimate the values with a positive bias of 75.7.
When analyzing the grouped \emph{Scale Variable}, a similar trend is observed, while the accuracy boosts to 67.6 for ChatGPT and 59.0 for Llama2.

In \emph{Category Variable}, ChatGPT significantly outperforms Llama2 with an accuracy of 77.2\% against 63.6\%.
ChatGPT's performance in Calculation variables also surpasses that of Llama2, with accuracies of 64.4\% and 56.5\%, respectively. 
The positive bias indicates a tendency in both models to underestimate the true values.

The \emph{Notes Variable} is exclusively evaluated using the Recall metric. 
Llama2 demonstrates a modestly better performance with a recall of 52.7\%, compared to ChatGPT's recall of 48.1\%. 
This suggests that Llama2 has a better capability in retrieving pertinent information.


